Wearable Haptics for Remote Social Walking

Walking is an essential activity for a healthy life, which becomes less tiring and more enjoyable if done together. Common difficulties we have in performing sufficient physical exercise, for instance the lack of motivation, can be overcome by exploiting its social aspect. However, our lifestyle sometimes makes it very difficult to find time together with others who live far away from us to go for a walk. In this paper we propose a novel system enabling people to have a 'remote social walk' by streaming the gait cadence between two persons walking in different places, increasing the sense of mutual presence. Vibrations provided at the users' ankles display the partner's sensation perceived during the heel-strike. In order to achieve the aforementioned goal in a two users experiment, we envisaged a four-step incremental validation process: i) a single walker has to adapt the cadence with a virtual reference generated by a software; ii) a single user is tasked to follow a predefined time varying gait cadence; iii) a leader-follower scenario in which the haptic actuation is mono-directional; iv) a peer-to-peer case with bi-directional haptic communication. Careful experimental validation was conducted involving a total of 50 people, which confirmed the efficacy of our system in perceiving the partners' gait cadence in each of the proposed scenarios.

==> final_submission - arxiv/figures/representativeExperiments.tex <==
\begin{figure*}
    \centering
    
    \begin{subfigure}{0.32\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figures/artificialLeader} 
        \caption{Artificial Leader}
        \label{fig:exp1}
    \end{subfigure} %
    \begin{subfigure}{0.32\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figures/leadFollow} 
        \caption{Human Leader}
        \label{fig:exp2}
    \end{subfigure} %
    \begin{subfigure}{0.32\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figures/p2p} 
        \caption{Peer-to-Peer}
        \label{fig:exp3}
    \end{subfigure}    
    \caption{\TL{In (a) we examined the human capability in entraining to an external rhythm generated by an algorithm. The suggested cadence could be either constant, as in the Artificial Constant Reference experiment (\sect\ref{SEC:VirtualReference}), or time-varying (\sect\ref{SEC:ExpArtificialLeader}). In (b) a representative frame of the \lq\lq Human Leader'' experiment (\sect\ref{SEC:ExpHumanLeader}) is depicted. The follower is asked to synchronize to the gait pace of another human using the proposed system. This experiment differs from the previous one since the human's stride duration is not regular, but features small unpredictable variations. Finally, in the \lq\lq Peer-to-peer'' configuration (c) we tested the bidirectional capability of our system (see \sect\ref{SEC:ExpP2P}). Both participants were sending each other their respective gait cadence (sensed by their anklet devices). 
The direction of the information is graphically represented by the arrows. }}
    \label{fig:manmade}
\end{figure*}

==> final_submission - arxiv/figures/setup.tex <==
\begin{figure}[t]
  \centering
\begin{subfigure}{.6\columnwidth}
  \centering
\includegraphics[width=0.9\columnwidth]{\MyPath/figures/bracelet_covered_2motors}\\
\includegraphics[width=0.9\columnwidth]{\MyPath/figures/bracelet_2motors_text}
\end{subfigure}%
\begin{subfigure}{.4\columnwidth}
  \centering
\includegraphics[width=0.9\columnwidth]{\MyPath/figures/setup2}
\end{subfigure}
\caption{Haptic cues are provided to the users via two vibrotactile interfaces placed on the ankles. The interfaces are composed of two vibrating motors (1) attached to an elastic band (3). A Li-Ion battery and an Arduino board are in~(2). \label{FIG:bracelet2Motors}
}
\label{fig:anklets}
\end{figure}


==> final_submission - arxiv/tablePercentage.tex <==
\begin{table}[]
\centering
\begin{adjustbox}{center, width=0.9\columnwidth}  % can also use \linewidth or sth. else
\footnotesize
\begin{tabular}{r|rrr|rrr|c}
\hline \hline
\textbf{Name}    & \multicolumn{3}{c|}{\textbf{Haptics}} & \multicolumn{3}{c|}{\textbf{Haptics + Secondary Task}} & \textbf{Note} \\ \hline
        & 2\%       & 4\%       & 6\%       & 2\%        & 4\%         & 6\%          & \\ \hline
User1   & 66,32     & 99,05     & 100,00    & 47,36      & 84,88       & 92,59        & \\ 
User2   & 89,06     & 100,00    & 100,00    & 88,19      & 100,00      & 100,00       & $\bigstar$\\ 
User3   & 78,90     & 98,00     & 99,80     & 28,85      & 78,19       & 99,60        & \\ 
User4   & 47,35     & 98,83     & 100,00    & 78,66      & 100,00      & 100,00       &  \\ 
User5   & 91,13     & 100,00    & 100,00    & 38,88      & 77,34       & 87,43        & \\ 
User6   & 81,52     & 96,53     & 100,00    & 55,82      & 93,43       & 100,00       & \\ 
User7   & 89,95     & 99,69     & 100,00    & 36,91      & 86,95       & 100,00       & \\ 
User8   & 94,78     & 100,00    & 100,00    & 25,19      & 78,78       & 100,00       & \\ 
User9   & 76,98     & 98,47     & 99,96     & 44,80      & 80,38       & 92,29        & \\ 
User10  & 80,38     & 100,00     & 100,00    & 67,61      & 100,00      & 100,00       & $\bigstar$ \\ 
User11  & 66,58     & 94,41     & 100,00    & 0,00       & 4,20        & 39,82        & \\ 
User12  & 41,50     & 94,30     & 99,52     & 34,45      & 98,54       & 100,00       & \\ 
User13  & 83,28     & 100,00    & 100,00    & 48,96      & 97,32       & 100,00       & \\ 
User14  & 78,77     & 94,68    & 100,00    & 19,07      & 62,93       & 97,33        & \\ 
User15  & 76,01     & 99,50     & 100,00    & 76,01      & 99,52       & 100,00       & \\ 
User16  & 90,76     & 100,00    & 100,00    & 47,63      & 84,67       & 94,27        & \\ 
User17  & 77,10     & 98,56     & 100,00    & 49,64      & 81,36       & 93,68        & \\ 
User18  & 88,35     & 99,60     & 100,00    & 50,88      & 92,36       & 100,00       & \\ 
User19  & 73,78     & 88,66     & 99,09     & 53,58      & 88,04       & 91,48        & \\ 
User20  & 72,27     & 100,00    & 100,00    & 39,28      & 82,75       & 95,68        & \\ \hline
%User21  & 72,04     & 100,00    & 100,00    & 42,75      & 78,49       & 90,34        & \\ \hline
%User22  & 69,23     & 97,05     & 100,00    & 31,07     & 81,73       & 87,16        & \\ \hline
%User23  & 72,77     & 97,70     & 100,00    & 40,84     & 85,03       & 91,00        & \\ \hline
%User24  & 79,62     & 94,48     & 100,00    & 50,14     & 76,52       & 94,95        & \\ \hline
%User25  & 83,62     & 100,00    & 100,00    & 50,25      & 80,72       & 100,00       & \\ \hline
%User26  & 80,73     & 93,61     & 100,00    & 44,55      & 76,84       & 100,00       & \\ \hline
%User27  & 77,62     & 97,76    	& 100,00    & 35,12      & 79,32       & 96,79        & \\ \hline
%User28  & 78,05     & 98,56    	& 100,00    & 48,69      & 76,19       & 93,87        & \\ \hline
%User29  & 74,83     & 100,00    & 100,00    & 36,28      & 76,77       & 100,00       & \\ \hline
%User30  & 81,51     & 100,00    & 100,00    & 49,04      & 89,70       & 100,00       & \\ \hline

%\multicolumn{7}{c}{}\\ 

%\hline 

%\textbf{Mean} & \textbf{77,24}     & \textbf{98,01}     & \textbf{99,92}     & \textbf{46,59}      & \textbf{83,58}       & \textbf{94,21 }      \\ 
\hline
\textbf{Percentile 25} & \textbf{72.65} & \textbf{96.90}  & \textbf{100.00} & \textbf{35.07} & \textbf{79.18} & \textbf{92.86}  \\
\textbf{Percentile 50} & \textbf{78.84} & \textbf{99.28}  & \textbf{100.00} & \textbf{47.50} & \textbf{85.92} & \textbf{99.80}  \\
\textbf{Percentile 75} & \textbf{88.88} & \textbf{100.00} & \textbf{100.00} & \textbf{55.26} & \textbf{98.24} & \textbf{100.00} \\


%\textbf{STD}     & \textbf{13,80}     & \textbf{2,95}      & \textbf{0,23}      & \textbf{20,89}      & \textbf{21,17}       & \textbf{13,37}       \\ 
\hline \hline
\end{tabular}
\end{adjustbox}
\caption{For each user are reported the percentages of trial duration during which the participant aligned his cadence with the reference rhythm, grouped wrt the considered error bands. Please notice that users tagged with $\bigstar$ are the two high level music players.}
\label{TABLE:synchronization_intervals}
\end{table}


==> final_submission - arxiv/table_botFollower.tex <==
\begin{table}[]
\centering
\begin{adjustbox}{center, width=\columnwidth}  % can also use \linewidth or sth. else
\begin{tabular}{cccc} 
\hline \hline 
\textbf{User} & \textbf{\begin{tabular}[c]{@{}c@{}}Baseline\\ Stride Duration\\ (ms/stride)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Time for\\ Alignment\\ (s)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Alignment\\ Percentage\\ \%\end{tabular}} \\
\hline
U1  & 1206 & 4.0 & 100\% \\
U2  & 1336 & 4.7 & 100\% \\
U3  & \ 955  & 3.6 & \ 99\%  \\
U4  & \ 998  & 1.0 & \ 97\%  \\
U5  & \ 905  & 3.8 & \ 99\%  \\
U6  & \ 920  & 0.3 & \ 98\%  \\
U7  & \ 879  & 4.8 & \ 99\%  \\
U8  & 1006 & 2.9 &  \ 98\%  \\
U9  & 1060 & 4.2 & \ 95\%  \\
U10 & \ 986  & 5.6 & 100\% \\
U11 & \ 881  & 4.5 & \ 99\%  \\
U12 & \ 885  & 4.5 & \ 99\%  \\
U13 & \ 980  & 1.5 & \ 99\%  \\
U14 & 1009 & 4.3 & \ 98\%  \\
U15 & 1168 & 1.5 & \ 94\% \\
U16 & 1077 & 5.5 & \ 99\%  \\
U17 & \ 961  & 2.1 & \ 98\%  \\
U18 & 1058 & 2.5 & 100\% \\
U19 & 1297 & 2.7 &\  99\%  \\
U20 & 1251 & 5.4 & \ 99\% \\
%\hline
%\textbf{AVERAGE} & & \textbf{3.5}  & \textbf{ 98.45\%} 
\hline \hline
\end{tabular}                                   
\end{adjustbox}
\caption{Artificial Leader. For each user we report data from the experimental validation. The first column details the user's comfortable cadence (\iec  cadence without haptic suggestion). In the second column we report the total time needed to align the actual cadence to the displayed one. The last column describes the percentage of time in which the subject was aligned with the suggested rhythm.}
\label{tab:botFollower}
\end{table}

==> final_submission - arxiv/table_constant_rhythm.tex <==
\TL{
\begin{table}[]
\centering
\begin{adjustbox}{center, width=0.9\columnwidth}  
\begin{tabular}{cccccc}
\hline \hline 
\textbf{User} & \textbf{\begin{tabular}[c]{@{}c@{}}Baseline\\ Stride Dur.\\ (ms/stride)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Time for\\ Alignment\\ (-$10\%$) (s)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Alignment\\ Percentage\\(-$10\%$) \%\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Time for\\ Alignment\\ (+$10\%$) (s)\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Alignment\\ Percentage\\(+$10\%$) \%\end{tabular}}\\
\hline
U1 & \ 995  & 0.4 & 100.00 & 3.5 & \ 98.11 \\
U2 & 1146 & 1.3 & 100.00 & 1.5 & 100.00 \\
U3 & 1060 & 1.5 & \ 95.23 & 4.0 & \ 94.72 \\
U4 & 1021 & 2.6 & \ 95.09 & 3.1 & 100.00 \\
U5 & 1078 & 2.4 & 100.00 & 3.1 & 100.00 \\
U6 & \ 975  & 1.4 & 100.00 & 2.1 & \ 97.32 \\
U7 & 1107 & 2.6 & \ 97.34 & 1.8 & 100.00 \\
U8 & 1098 & 5.4 & 100.00 & 0.6 & \ 95.21 \\
U9 & 1100 & 1.7 & \ 97.66 & 1.9 & 100.00 \\
U10 & 1208 & 5.1 &\ 96.38 & 1.6 & \ 98.01 \\
%\hline
%\textbf{AVERAGE} & & & & & \\ 
\hline \hline
\end{tabular}
\end{adjustbox}
\caption{\TL{Data extracted from experimental data are listed in the table. The baseline stride duration represents the average cadence measured during the haptic-off trials. Time for alignment and Alignment percentages are then reported for fast ($-10\%$) and slow cadence condition ($+10\%$).}}
\label{tab:constant}
\end{table}
}

==> final_submission - arxiv/table_leaderFollower.tex <==
\begin{table*}[t]
\centering
\begin{adjustbox}{center, width=2\columnwidth}  % can also use \linewidth or sth. else
\begin{tabular}{cccccccc}
\hline \hline
\textbf{Leader} & \textbf{Follower} & \begin{tabular}[c]{@{}c@{}}\textbf{Leader B}\\ \textbf{Stride Duration}\\ \textbf{(ms/stride)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Follower B}\\ \textbf{Stride Duration}\\ (\textbf{ms/stride)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Mean H}\\ \textbf{Stride Duration}\\ \textbf{(ms/stride})\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{STD H}\\ \textbf{Stride Duration}\\ \textbf{(ms/stride)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Time for}\\ \textbf{Alignment}\\ \textbf{(s)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Alignment}\\ \textbf{Percentage}\\ \textbf{\%}\end{tabular} \\
\hline
U1	&	U2	&	1023	&	1141	&	1022	&	19	&	2.0	&	97\%	\\
U3	&	U4	&	1145	&	1035	&	1151	&	21	&	4.4	&	99\%	\\
U5	&	U6	&	1025	&	1136	&	1037	&	17	&	3.5	&	94\%	\\
U7	&	U8	&	1014	&	1081	&	1017	&	16	&	3.2	&	98\%	\\
U9	&	U10	&	1050	&	1082	&	1042	&	18	&	3.9	&	96\%	\\
U11	&	U12	&	1113	&	1106	&	1110	&	17	&	3.2	&	99\%	\\
U13	&	U14	& 	1020	&	1070	&	1024	&	16	&	2.5	&	95\%	\\
U15	&	U16	&	1086	&	1030	&	1078	&	20	&	3.9	&	98\%	\\
U17	&	U18	&	1055	&	1101	&	1059	&	23	&	3.0	&	94\%	\\
U19	&	U20	&	1018	&	1081	&	1030	&	20	&	3.5	&	98\%	\\
\hline
\multicolumn{2}{c}{\textbf{AVERAGE}} & & & & \textbf{18.7}& \textbf{3.31}  & \textbf{96.8\%} \\ \hline \hline
\end{tabular}
\end{adjustbox}
\caption{Human Leader. The table details data regarding the experiment with the human leader, where \textbf{B} and \textbf{H} stand for baseline and haptic-on condition, respectively. Mean cadences estimated in the first part of the trial (without haptics) are reported for both the users, and compared to the average walking rhythm during the phase with the haptic stimulation (Mean H). It is important to notice that the standard deviation of the mean cadence during the phase with haptic stimulation is comparable with the variability registered in the comfortable cadence walking.}
\label{tab:LeaderFollower}
\end{table*}

==> final_submission - arxiv/table_masterMaster.tex <==
\begin{table*}[]
\centering
\begin{adjustbox}{center, width=1.85\columnwidth}  % can also use \linewidth or sth. else
\begin{tabular}{cccccccccccc}
\hline \hline	
\multicolumn{1}{l}{\textbf{User1}} & \multicolumn{1}{l}{\textbf{User2}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}User1 B \\  Stride Duration \\ (ms/stride)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}User2 B \\ Stride Duration\\  (ms/stride)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mean H \\ Stride Duration\\ (ms/stride)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}STD H\\ Stride Duration\\ (ms/stride)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Time for \\ Alignment \\(s)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} Alignment \\ percentage\\ \%\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}User1 \\ Variation \\ \% \end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}User2 \\ Variation\\ \% \end{tabular}}} \\
\hline 
U1  & U2  & 1082 & 1158 & 1136 & 18 & 3.6 & 95\% & 5\% & 2\% \\
U3  & U4  & 1060 & 1002 & 1023 & 25 & 5.2 & 96\% & 4\% & 2\% \\
U5  & U6  & 1139 & 1136 & 1190 & 32 & 4.2 & 96\% & 4\% & 5\% \\
U7  & U8  & 1004 & 1070 & 1083 & 25 & 2.8 & 91\% & 7\% & 1\% \\
U9  & U10 & 1039 & \ 982  & 1046 & 31 & 1.1 & 92\% & 1\% & 6\% \\
U11 & U12 & 1067 & 1047 & 1090 & 35 & 5.6 & 93\% & 2\% & 4\% \\
U13 & U14 & 996  & 1167 & 1087 & 33 & 11.6 & 99\% & 8\% & 7\% \\
U15 & U16 & 1102 & 1119 & 1145 & 33 & 7.3 & 86\% & 4\% & 2\% \\
U17 & U18 & 1032 & 1103 & 1067 & 22 & 4.9 & 99\% & 3\% & 3\% \\
U19 & U20 & 1082 & 1197 & 1116 & 24 & 2.9 & 98\% & 3\% & 7\% \\
% &	&	&	&	&	&	&	&	&	&	&	\\ 
\hline
\multicolumn{2}{c}{\textbf{AVERAGE}	}	&	&	&	& \textbf{28}	& \textbf{4.9}	& \textbf{94.5\%}	& \textbf{4.1\%}	& \textbf{3.9\%}	\\ \hline \hline 
\end{tabular}
\end{adjustbox}
\caption{Peer-to-peer. The table details data regarding the final experiment, where \textbf{B} and \textbf{H} stand for baseline and haptic-on condition, respectively. Mean cadences estimated in the first part of the trial (without haptics) are reported for both the users, and compared to the average walking rhythm during the phase with the haptic stimulation (Mean H). Also in this experiment is important to notice that the standard deviation of the mean cadence during the phase with haptic stimulation is comparable with the variability registered in the comfortable cadence walking.}
\label{tab:peerToPeer}
\end{table*}
